Matrix-Based Characterization of the Motion and Wrench Uncertainties in Robotic Manipulators

Characterization of the uncertainty in robotic manipulators is the focus of this paper. Based on the random matrix theory (RMT), we propose uncertainty characterization schemes in which the uncertainty is modeled at the macro (system) level. This is different from the traditional approaches that model the uncertainty in the parametric space of micro (state) level. We show that perturbing the system matrices rather than the state of the system provides unique advantages especially for robotic manipulators. First, it requires only limited statistical information that becomes effective when dealing with complex systems where detailed information on their variability is not available. Second, the RMT-based models are aware of the system state and configuration that are significant factors affecting the level of uncertainty in system behavior. In this study, in addition to the motion uncertainty analysis that was first proposed in our earlier work, we also develop an RMT-based model for the quantification of the static wrench uncertainty in multi-agent cooperative systems. This model is aimed to be an alternative to the elaborate parametric formulation when only rough bounds are available on the system parameters. We discuss that how RMT-based model becomes advantageous when the complexity of the system increases. We perform experimental studies on a KUKA youBot arm to demonstrate the superiority of the RMT-based motion uncertainty models. We show that how these models outperform the traditional models built upon Gaussianity assumption in capturing real-system uncertainty and providing accurate bounds on the state estimation errors. In addition, to experimentally support our wrench uncertainty quantification model, we study the behavior of a cooperative system of mobile robots. It is shown that one can rely on less demanding RMT-based formulation and yet meets the acceptable accuracy.

==> Fig_CoopSysExmp.tex <==
%----------------------------------------
\begin{figure}[htb!]
\centering
\begin{minipage}[t]{0.27\textwidth}
\includegraphics[trim=70 50 50 70, clip, scale=0.17]{AerialTow.pdf}

\hspace{0.55in}(a)
\end{minipage}% 
%.....................................
\hspace{-0.4in}
%.....................................
\begin{minipage}[t]{0.27\textwidth}
\includegraphics[trim=50 50 50 70, clip, scale=0.17]{HangWindTun.pdf} 

\hspace{0.65in}(b)
\end{minipage}%
\caption{Representative examples of the cooperative systems: (a) aerial towing/suspension using flying robots; (b) airplane hangar where bases can be re-adjusted along the rails.}
\label{Exmpls}
\end{figure}
%----------------------------------------

==> Fig_Histogrms.tex <==
%----------------------------------------------------------------------------
\begin{figure}[b!]
\centering
\includegraphics[trim=0 0 0 10, clip, scale=1]{ERRHist_Wrench.eps}
\caption{Error histograms. For 2000 samples of system state and parameters, the Euclidean distances (error) between the output wrench variances obtained by RMT-based model and those given by parametric model are calculated. 5 histograms with different colors correspond to 5 systems with different number of cables.}
\label{ErrWrnRMT}
\end{figure}
%----------------------------------------------------------------------------

==> Fig_KinKUKAEstim.tex <==
%----------------------------------------
\begin{figure}[b!]
\centering
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{KinImgKUKA150.eps}

\hspace{0.35in}(a)
\end{minipage}% 
%.....................................
\hspace{-0.4in}
%.....................................
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{KinImgKUKA250.eps} 

\hspace{0.6in}(b)
\end{minipage}%

\caption{Estimation of the joint angles of the KUKA youBot using Kinect measurement. (a) is the initial and final configuration and (b) shows the most extended configuration while tracking the desired trajectory. In order to improve the estimation of the joint angles, we allowed the length of the segments to change in a certain range.}
\label{KinOptFig}
\end{figure}

==> Fig_KinectNoiseChar.tex <==
%----------------------------------------
\begin{figure}
\centering
\begin{minipage}[t]{0.25\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{KinNoiseMean.eps}

\hspace{0.9in}(a)
\end{minipage}% 
%.....................................
%.....................................
\begin{minipage}[t]{0.25\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{KinNoiseSTD.eps} 

\hspace{0.9in}(b)
\end{minipage}%
\caption{Noise characteristics of the Kinect sensor.
%compared with OptiTrack data for 50 experimental trials. 
(a) shows the mean and (b) shows the standard deviation. It can be seen that Kinect noise is biased and its characteristics are time-varying.}
\label{MeanStdKinNoise}
\end{figure}
%----------------------------------------

==> Fig_PartFilt.tex <==
\begin{figure*}[htb!]
\centering
\small{\begin{minipage}[t]{0.35\textwidth}
\center{\qquad $\bm{q}_{1}$}
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\center{\ $\bm{q}_{2}$}
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\center{\ $\bm{q}_{3}$}
\end{minipage}}\hfill\\
%**********************************************************
\begin{minipage}[t]{0.35\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltAddGaussq1.eps}
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltAddGaussq2.eps} 
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltAddGaussq3.eps} 
\end{minipage}\hfill\\
%**********************************************************
\begin{minipage}[t]{0.35\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltWishq1.eps}
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltWishq2.eps} 
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltWishq3.eps} 
\end{minipage}\hfill\\
%**********************************************************
\begin{minipage}[t]{0.35\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltGaussRMTq1.eps}
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltGaussRMTq2.eps} 
\end{minipage}\hfill
\begin{minipage}[t]{0.325\textwidth}
\includegraphics[trim=0 0 0 0, clip, scale=1]{PartFiltGaussRMTq3.eps} 
\end{minipage}\hfill\\

\caption{State estimation errors in particle filtering. First row shows the results corresponding to the additive Gaussian noise model. Second row shows the results corresponding to the RMT-based model with Wishart perturbation matrix. Third row corresponds to the RMT-based stochastic model based on Gaussian noise matrix. Red lines are the $1-\sigma$ error bounds and blue lines show the actual error.}
\label{PartFiltRes}
\end{figure*}
%---------------------------------------------------------------------------  
 

==> Fig_WrenchExprmnt.tex <==
%---------------------------------------------------------------------------
\begin{figure*}
\centering
\small{\begin{minipage}[t]{0.27\textwidth}
\center{Robots configuration\qquad }
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\center{Experimental observations}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\center{RMT-based model output  }
\end{minipage}}\\ \vspace{0.1in}
%**********************************************************
 \begin{minipage}[t]{0.27\textwidth}
\includegraphics[trim=125 50 125 0, clip, scale=0.25]{ExpSetup_TFMax.pdf}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=80 10 20 0, clip, scale=0.09]{ExpWrenchRes_3_Gamma0001.jpg} 
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=45 10 20 0, clip, scale=0.09]{RMT_WrnchRes_3_Gamma0001.jpg} 
\end{minipage}\\
%**********************************************************
\begin{minipage}[t]{0.27\textwidth}
\includegraphics[trim=125 50 125 0, clip, scale=0.25]{ExpSetup_FxVarMin.pdf}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=155 10 0 0, clip, scale=0.09]{ExpWrenchRes_3_Gamma1000.jpg} 
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=180 10 0 0, clip, scale=0.09]{RMT_WrnchRes_3_Gamma1000.jpg} 
\end{minipage}\\
%**********************************************************
\begin{minipage}[t]{0.27\textwidth}
\includegraphics[trim=125 50 125 0, clip, scale=0.25]{ExpSetup_FyVarMin.pdf}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=0 50 0 0, clip, scale=0.09]{ExpWrenchRes_3_Gamma0100.jpg} 
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\includegraphics[trim=0 50 0 0, clip, scale=0.09]{RMT_WrnchRes_3_Gamma0100.jpg} 
\end{minipage}

\caption{Experimental evaluation of RMT-based model in capturing the wrench (only force vector here) uncertainty. Three different configurations are shown in three rows. First column shows the configuration of the iRobots. The KS density of the (accurately) measured force is shown in second column. The KS density of the data points obtained from RMT-based model given by Eq.~(\ref{CovWNonPar}) is shown in the third column.}
\label{WrenchExprmnt}
\end{figure*}
